JLD: Perceptual Distance Through A Jacobian Lens

Image compression, restoration, and generation all require a way to measure how different two images look to a person. Pixel error ignores how people see, while the most accurate perceptual distances are typically fitted to human judgments, tying them to a fixed data and resolution. For example, when image resolution is doubled, the correlation of DISTS with human scores on TID2013 drops from 0.815 to 0.717. We introduce the Jacobian Lens Distance (JLD), which derives its perceptual geometry from a frozen vision encoder rather than from human labels. JLD combines the locality of early patch features with the perceptual sensitivity captured by later encoder representations. Specifically, we use the encoder Jacobian to identify directions in the early feature space that most strongly affect the encoder output, producing a fixed metric tensor, $E[J^\top J]$, which we call the Jacobian lens. The lens is fitted only once from 100 unlabeled images, taking about 35 seconds. Locally, this construction defines a pullback metric in pixel space, giving JLD a clear geometric interpretation that can be directly analyzed on real images. Across four standard perceptual databases, JLD achieves state-of-the-art performance and consistently outperforms LPIPS, DISTS, PieAPP, and DreamSim. JLD is also robust to changes in image resolution, on TID2013, its lens-term correlation remains nearly unchanged when the resolution is doubled, decreasing only from 0.850 to 0.845. We further introduce JLD-fast, which is $4\times$ faster than LPIPS-VGG while achieving a mean correlation of 0.911. Finally, JLD naturally extends to video, reaching a correlation of 0.786 on Waterloo IVC 4K compared with 0.611 for VMAF.

==> sections/ai_use.tex <==
\section*{The Use of Large Language Models (LLMs)}\phantomsection\label{sec:llm}
During the preparation of this work, the authors used ChatGPT (OpenAI) to assist with text editing and formatting the paper. ChatGPT was also used as a coding assistant to implement some of the result analysis and figure scripts in Python. All suggestions, text and code produced with its help were reviewed, edited and verified by the authors, who take full responsibility for the content of the paper. The ideas, method, experimental design and results are the original work of the authors.


==> sections/figs/app_fig_study_trials.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{v22/app_study_trials.pdf}
% Source: scripts/v22/fig_study.py; results/study_trials.csv in file order; counts in figures/v22/app_study_trials_numbers.json.
% \caption{Every study trial in protocol order, aligned across metrics.
% MAD and gMAD trials use earlier lens-only scores; rated-image trials use full \name{}.
% \name{} has 12 ties; DISTS has 10 ties and no score on four gMAD trials.}
\caption{Every study trial in protocol order, aligned across metrics. MAD and gMAD trials use earlier lens-only scores; rated-image trials use full \name{}.}
\label{fig:study-coverage}
\end{figure}


==> sections/figs/fig_chroma.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{v22/fig_chroma.pdf}
% Source: figures/v22/fig_chroma_numbers.json; MOS, D_ws (unfiltered) and D_ws_fe (pre-filtered) from results/explore/e06_tid2013_chroma_s2.csv;
% PSNR, LPIPS-VGG, DISTS from results/baselines_fr_tid2013_crop.csv; maps from figures/v22/visuals_maps.npz. Win rates: win_rates in scripts/v22/visuals.py.
% \caption{TID2013 colour-channel noise has 2.8\,dB lower PSNR than Gaussian noise yet higher MOS; the unfiltered lens scores it as worse (0.153 against 0.133), and the chroma pre-filter reverses the order (0.100 against 0.117).
% Maps share one colour scale and exclude the CLS term.
% Bars give each method's win rate: the share of 623 same-scene TID2013 pairs of colour and Gaussian noise that it orders as humans do.}
\caption{TID2013 colour-channel noise against Gaussian noise: the chroma pre-filter reverses the unfiltered lens's order to match MOS. Maps share one colour scale and exclude the CLS term. Bars: share of 623 same-scene pairs of the two noise types ordered as humans do.}
\label{fig:chroma}
\end{figure}


==> sections/figs/fig_native.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{v22/fig_native.pdf}
% Source: figures/v22/fig_native_numbers.json; MOS and native DISTS/LPIPS preferences from figures/v5/fig4_qual_numbers.json (KADID-10k I09);
% maps and per-size JLD scores from figures/v22/visuals_maps.json (released package, CPU; native scores reproduce the recorded values). Script scripts/v22/visuals.py.
% \caption{On a matched-PSNR KADID-10k pair, humans and \name{} prefer JPEG compression (A) to a colour shift (B) at every input size, while DISTS and LPIPS prefer B at native size.
% Maps share one colour scale; the yellow box marks the enlarged detail.}
\caption{A matched-PSNR KADID-10k pair: humans and \name{} prefer JPEG compression (A) to a colour shift (B) at every input size; DISTS and LPIPS prefer B at native size.}
\label{fig:native}
\end{figure}


==> sections/figs/fig_qual_main.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{v22/fig_qual_main.pdf}
% Source: figures/v22/fig_qual_main_numbers.json; I04 and I05 from figures/v5/fig9_gallery_numbers.json; I07 and I75 from
% results/explore/e06_{tid2013,kadid10k_test}_chroma_s2.csv and results/baselines_fr_*_crop.csv, maps from figures/v22/visuals_maps.npz. Script scripts/v22/visuals.py.
% \caption{Four pairs at matched PSNR (within 0.02\,dB) where humans and \name{} prefer the top image and DISTS and LPIPS-VGG prefer the bottom one.
% Each detail sits beside its \name{} map on one shared square-root colour scale, with the \name{} score; Figure~\ref{fig:gallery} shows more pairs.}
\caption{Four pairs at matched PSNR where humans and \name{} prefer the top image and DISTS and LPIPS-VGG the bottom one. Each detail sits beside its \name{} map (one square-root colour scale).}
\label{fig:qual-main}
\end{figure}


==> tables/app_bootstrap.tex <==
% Generated by scripts/v23/bench_bootstrap_table.py from figures/v23/bench_bootstrap_numbers.json
% (scripts/v23/bench_bootstrap.py: 1,000 reference-level bootstrap draws per dataset, seed 0).
% v23.3 (D2): the mean-of-four column moved to the text of app:moved-results; the table is a wraptable there.
\begin{wraptable}{r}{0.48\linewidth}
\vspace{-12pt}
\centering\small
\setlength{\tabcolsep}{2.5pt}
\caption{\srcc{} of \name{} minus each method (1{,}000 reference bootstrap draws). Italic: interval contains zero; grey: below zero.}
\label{tab:app_bootstrap}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Method & TID & CSIQ & LIVE & KADID \\
\midrule
\namefast{} & \textit{$+0.002$} & $+0.015$ & $+0.019$ & $+0.021$ \\
VSI & \textcolor{gray}{$-0.018$} & $+0.031$ & $+0.015$ & $+0.015$ \\
DeepWSD & $+0.021$ & $+0.012$ & $+0.009$ & $+0.010$ \\
DeepDC & $+0.061$ & $+0.017$ & $+0.014$ & \textcolor{gray}{$-0.008$} \\
FSIM & $+0.026$ & $+0.040$ & \textit{$-0.001$} & $+0.039$ \\
GMSD & $+0.072$ & $+0.014$ & \textit{$+0.004$} & $+0.043$ \\
DISTS & $+0.059$ & $+0.028$ & $+0.010$ & \textit{$+0.006$} \\
PieAPP & \textit{$+0.033$} & $+0.074$ & $+0.046$ & $+0.027$ \\
DreamSim & $+0.065$ & $+0.059$ & $+0.054$ & $+0.041$ \\
LPIPS-VGG & $+0.207$ & $+0.088$ & $+0.032$ & $+0.168$ \\
TOPIQ-FR & \textcolor{gray}{$-0.040$} & \textit{$+0.003$} & \textcolor{gray}{$-0.012$} & \textcolor{gray}{$-0.094$} \\
\bottomrule
\end{tabular}
\vspace{-8pt}
\end{wraptable}


==> tables/app_cost.tex <==
% Generated by scripts/70_tables_v5.py; do not edit by hand.
% Protocol: results/notes/cost.md; batch=1, CPU threads=12, A100, 512x384 except IEM 256x256.
% v23.5 P2: compact float with the caption beside the table (was \begin{table}[tbp], \small, full width, caption on top).
% v23.6 P6: no side caption; a wrapped table with the caption on top.
% \begin{table}[tb]
% \begin{minipage}[c]{0.62\linewidth}
% v23.8 (L8): the 24-line wraptable forced a large gap before its section; it is now a normal float (same rows).
\begin{table}[tb]
\centering\footnotesize
\captionsetup{font=footnotesize,skip=2pt}
\caption{Cost per image pair. Violet: ours; grey: trained on human judgements. \textbf{Bold} and \underline{underlining} mark the lowest and second-lowest cost in each numeric column.}
\label{tab:app_cost}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.03}
% \caption{Cost per image pair. Violet: ours; grey: fitted on human judgements; white: other baselines.}  (moved beside the table)
% \label{tab:app_cost}  (moved beside the table)
\colorlet{humanJudgements}{gray!7}
\definecolor{ourMetrics}{HTML}{F3EFF8}
\begin{tabular*}{0.72\linewidth}{@{\extracolsep{\fill}}lrrrrr@{}}
\toprule
Metric & GFLOPs & GPU ms & CPU ms & \shortstack{Peak GPU\\MB} & Labels \\
\midrule
% Cell gflops_per_pair=10.7; exact=10.720791552; source: results/cost.csv:2, metric=jld, column=gflops_per_pair.
% Cell gpu_ms_per_pair=2.5; exact=2.525739546399564; source: results/cost.csv:2, metric=jld, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=29.8; exact=29.782272991724312; source: results/cost.csv:2, metric=jld, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=114.0; exact=113.99755859375; source: results/cost.csv:2, metric=jld, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:2, metric=jld, column=human_labels_used.
\rowcolor{ourMetrics}\namefast{} & 10.7 & 2.5 & 29.8 & 114.0 & 0 \\
% Cell gflops_per_pair=118.5; exact=118.467293184; source: results/cost.csv:3, metric=jld_full12, column=gflops_per_pair.
% Cell gpu_ms_per_pair=12.2; exact=12.249739957042038; source: results/cost.csv:3, metric=jld_full12, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=253.7; exact=253.668243996799; source: results/cost.csv:3, metric=jld_full12, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=115.4; exact=115.43505859375; source: results/cost.csv:3, metric=jld_full12, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:3, metric=jld_full12, column=human_labels_used.
\rowcolor{ourMetrics}\name{} & 118.5 & 12.2 & 253.7 & 115.4 & 0 \\
% Cell gflops_per_pair=$<$0.1; exact=0.0; source: results/cost.csv:4, metric=psnr, column=gflops_per_pair.
% Cell gpu_ms_per_pair=1.4; exact=1.4140065177343786; source: results/cost.csv:4, metric=psnr, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=1.1; exact=1.112711033783853; source: results/cost.csv:4, metric=psnr, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=9.0; exact=9.0; source: results/cost.csv:4, metric=psnr, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:4, metric=psnr, column=human_labels_used.
PSNR & \textbf{$<$0.1} & \underline{1.4} & \textbf{1.1} & \textbf{9.0} & 0 \\
% Cell gflops_per_pair=0.2; exact=0.234252968; source: results/cost.csv:5, metric=ssim, column=gflops_per_pair.
% Cell gpu_ms_per_pair=2.7; exact=2.678551943972707; source: results/cost.csv:5, metric=ssim, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=92.6; exact=92.56007801741362; source: results/cost.csv:5, metric=ssim, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=34.5; exact=34.529296875; source: results/cost.csv:5, metric=ssim, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:5, metric=ssim, column=human_labels_used.
SSIM & \underline{0.2} & 2.7 & 92.6 & 34.5 & 0 \\
% Cell gflops_per_pair=0.3; exact=0.303561768; source: results/cost.csv:6, metric=ms_ssim, column=gflops_per_pair.
% Cell gpu_ms_per_pair=5.1; exact=5.118806497193873; source: results/cost.csv:6, metric=ms_ssim, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=119.1; exact=119.14976697880776; source: results/cost.csv:6, metric=ms_ssim, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=34.5; exact=34.52978515625; source: results/cost.csv:6, metric=ms_ssim, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:6, metric=ms_ssim, column=human_labels_used.
MS-SSIM & 0.3 & 5.1 & 119.1 & 34.5 & 0 \\
% Cell gflops_per_pair=$<$0.1; exact=0.005308416; source: results/cost.csv:7, metric=fsim, column=gflops_per_pair.
% Cell gpu_ms_per_pair=22.8; exact=22.846897481940687; source: results/cost.csv:7, metric=fsim, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=60.6; exact=60.573618044145405; source: results/cost.csv:7, metric=fsim, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=46.2; exact=46.18798828125; source: results/cost.csv:7, metric=fsim, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:7, metric=fsim, column=human_labels_used.
FSIM & \textbf{$<$0.1} & 22.8 & 60.6 & 46.2 & 0 \\
% Cell gflops_per_pair=$<$0.1; exact=0.015335424; source: results/cost.csv:8, metric=vsi, column=gflops_per_pair.
% Cell gpu_ms_per_pair=9.9; exact=9.872902475763112; source: results/cost.csv:8, metric=vsi, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=39.8; exact=39.776562014594674; source: results/cost.csv:8, metric=vsi, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=48.7; exact=48.650390625; source: results/cost.csv:8, metric=vsi, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:8, metric=vsi, column=human_labels_used.
VSI & \textbf{$<$0.1} & 9.9 & 39.8 & 48.7 & 0 \\
% Cell gflops_per_pair=$<$0.1; exact=0.011403264; source: results/cost.csv:9, metric=gmsd, column=gflops_per_pair.
% Cell gpu_ms_per_pair=2.6; exact=2.5983754894696176; source: results/cost.csv:9, metric=gmsd, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=7.3; exact=7.331099011935294; source: results/cost.csv:9, metric=gmsd, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=18.6; exact=18.625; source: results/cost.csv:9, metric=gmsd, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:9, metric=gmsd, column=human_labels_used.
GMSD & \textbf{$<$0.1} & 2.6 & 7.3 & \underline{18.6} & 0 \\
% Cell gflops_per_pair=$<$0.1; exact=0.017856; source: results/cost.csv:10, metric=mad, column=gflops_per_pair.
% Cell gpu_ms_per_pair=247.9; exact=247.87814100272956; source: results/cost.csv:10, metric=mad, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=1,721.3; exact=1721.3351769605651; source: results/cost.csv:10, metric=mad, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=649.2; exact=649.15478515625; source: results/cost.csv:10, metric=mad, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:10, metric=mad, column=human_labels_used.
MAD & \textbf{$<$0.1} & 247.9 & 1,721.3 & 649.2 & 0 \\
% Cell gflops_per_pair=$<$0.1; exact=0.049952464; source: results/cost.csv:11, metric=nlpd, column=gflops_per_pair.
% Cell gpu_ms_per_pair=15.6; exact=15.560497005935758; source: results/cost.csv:11, metric=nlpd, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=27.1; exact=27.145628002472222; source: results/cost.csv:11, metric=nlpd, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=21.6; exact=21.60009765625; source: results/cost.csv:11, metric=nlpd, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:11, metric=nlpd, column=human_labels_used.
NLPD & \textbf{$<$0.1} & 15.6 & 27.1 & 21.6 & 0 \\
% Cell gflops_per_pair=1.7; exact=1.729021872; source: results/cost.csv:12, metric=vif, column=gflops_per_pair.
% Cell gpu_ms_per_pair=54.0; exact=53.98199800401926; source: results/cost.csv:12, metric=vif, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=126.6; exact=126.61413103342056; source: results/cost.csv:12, metric=vif, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=54.8; exact=54.83642578125; source: results/cost.csv:12, metric=vif, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:12, metric=vif, column=human_labels_used.
VIF & 1.7 & 54.0 & 126.6 & 54.8 & 0 \\
% Cell gflops_per_pair=240.6; exact=240.582918144; source: results/cost.csv:13, metric=lpips_vgg, column=gflops_per_pair.
% Cell gpu_ms_per_pair=10.9; exact=10.914095502812415; source: results/cost.csv:13, metric=lpips_vgg, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=418.5; exact=418.4992600930855; source: results/cost.csv:13, metric=lpips_vgg, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=532.3; exact=532.2646484375; source: results/cost.csv:13, metric=lpips_vgg, column=peak_gpu_MB.
% Cell human_labels_used=484,000; exact=484000; source: results/cost.csv:13, metric=lpips_vgg, column=human_labels_used.
\rowcolor{humanJudgements}LPIPS-VGG & 240.6 & 10.9 & 418.5 & 532.3 & 484,000 \\
% Cell gflops_per_pair=10.9; exact=10.861507584; source: results/cost.csv:14, metric=lpips_alex, column=gflops_per_pair.
% Cell gpu_ms_per_pair=3.7; exact=3.676026011817157; source: results/cost.csv:14, metric=lpips_alex, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=34.1; exact=34.0727650327608; source: results/cost.csv:14, metric=lpips_alex, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=63.0; exact=63.02294921875; source: results/cost.csv:14, metric=lpips_alex, column=peak_gpu_MB.
% Cell human_labels_used=484,000; exact=484000; source: results/cost.csv:14, metric=lpips_alex, column=human_labels_used.
\rowcolor{humanJudgements}LPIPS-Alex & 10.9 & 3.7 & 34.1 & 63.0 & 484,000 \\
% Cell gflops_per_pair=240.7; exact=240.747282432; source: results/cost.csv:15, metric=dists, column=gflops_per_pair.
% Cell gpu_ms_per_pair=9.9; exact=9.936597023624929; source: results/cost.csv:15, metric=dists, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=415.0; exact=415.02451710402966; source: results/cost.csv:15, metric=dists, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=340.7; exact=340.6953125; source: results/cost.csv:15, metric=dists, column=peak_gpu_MB.
% Cell human_labels_used=484,000; exact=484000; source: results/cost.csv:15, metric=dists, column=human_labels_used.
\rowcolor{humanJudgements}DISTS & 240.7 & 9.9 & 415.0 & 340.7 & 484,000 \\
% Cell gflops_per_pair=385.7; exact=385.679253504; source: results/cost.csv:16, metric=pieapp, column=gflops_per_pair.
% Cell gpu_ms_per_pair=16.5; exact=16.537297051399946; source: results/cost.csv:16, metric=pieapp, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=797.0; exact=797.0107579603791; source: results/cost.csv:16, metric=pieapp, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=1,005.5; exact=1005.51123046875; source: results/cost.csv:16, metric=pieapp, column=peak_gpu_MB.
% Cell human_labels_used=2,300,000; exact=2300000; source: results/cost.csv:16, metric=pieapp, column=human_labels_used.
\rowcolor{humanJudgements}PieAPP & 385.7 & 16.5 & 797.0 & 1,005.5 & 2,300,000 \\
% Cell gflops_per_pair=326.4; exact=326.356697088; source: results/cost.csv:17, metric=deepdc, column=gflops_per_pair.
% Cell gpu_ms_per_pair=16.1; exact=16.072013997472823; source: results/cost.csv:17, metric=deepdc, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=509.6; exact=509.5683719264344; source: results/cost.csv:17, metric=deepdc, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=325.2; exact=325.15478515625; source: results/cost.csv:17, metric=deepdc, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:17, metric=deepdc, column=human_labels_used.
DeepDC & 326.4 & 16.1 & 509.6 & 325.2 & 0 \\
% Cell gflops_per_pair=212.2; exact=212.154212352; source: results/cost.csv:18, metric=dreamsim, column=gflops_per_pair.
% Cell gpu_ms_per_pair=51.3; exact=51.26894399290904; source: results/cost.csv:18, metric=dreamsim, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=549.6; exact=549.6234609745443; source: results/cost.csv:18, metric=dreamsim, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=1,041.9; exact=1041.8583984375; source: results/cost.csv:18, metric=dreamsim, column=peak_gpu_MB.
% Cell human_labels_used=20,000; exact=20000; source: results/cost.csv:18, metric=dreamsim, column=human_labels_used.
\rowcolor{humanJudgements}DreamSim & 212.2 & 51.3 & 549.6 & 1,041.9 & 20,000 \\
% Cell gflops_per_pair=60.2; exact=60.189179904; source: results/cost.csv:19, metric=deepwsd, column=gflops_per_pair.
% Cell gpu_ms_per_pair=13.5; exact=13.5155440075323; source: results/cost.csv:19, metric=deepwsd, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=442.6; exact=442.63165502343327; source: results/cost.csv:19, metric=deepwsd, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=709.3; exact=709.29443359375; source: results/cost.csv:19, metric=deepwsd, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:19, metric=deepwsd, column=human_labels_used.
DeepWSD & 60.2 & 13.5 & 442.6 & 709.3 & 0 \\
% Cell gflops_per_pair=0.3; exact=0.339738624; source: results/cost.csv:20, metric=lasi, column=gflops_per_pair.
% Cell gpu_ms_per_pair=377.6; exact=377.6092884945683; source: results/cost.csv:20, metric=lasi, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=13,554.5; exact=13554.450307041408; source: results/cost.csv:20, metric=lasi, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=2,683.7; exact=2683.68896484375; source: results/cost.csv:20, metric=lasi, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:20, metric=lasi, column=human_labels_used.
LASI & 0.3 & 377.6 & 13,554.5 & 2,683.7 & 0 \\
% Cell gflops_per_pair=4,999.1; exact=4999.11643136; source: results/cost.csv:21, metric=iem, column=gflops_per_pair.
% Cell gpu_ms_per_pair=725.7; exact=725.7345230318606; source: results/cost.csv:21, metric=iem, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=22,766.5; exact=22766.52321300935; source: results/cost.csv:21, metric=iem, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=5,434.2; exact=5434.16259765625; source: results/cost.csv:21, metric=iem, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost.csv:21, metric=iem, column=human_labels_used.
IEM & 4,999.1 & 725.7 & 22,766.5 & 5,434.2 & 0 \\
% Cell gflops_per_pair=1.0; exact=0.973430784; source: results/cost_tiers.csv:2, metric=jld_lin, column=gflops_per_pair.
% Cell gpu_ms_per_pair=0.7; exact=0.6615369929932058; source: results/cost_tiers.csv:2, metric=jld_lin, column=gpu_ms_per_pair.
% Cell cpu_ms_per_pair=6.2; exact=6.238780915737152; source: results/cost_tiers.csv:2, metric=jld_lin, column=cpu_ms_per_pair.
% Cell peak_gpu_MB=112.3; exact=112.30224609375; source: results/cost_tiers.csv:2, metric=jld_lin, column=peak_gpu_MB.
% Cell human_labels_used=0; exact=0; source: results/cost_tiers.csv:2, metric=jld_lin, column=human_labels_used.
\rowcolor{ourMetrics}\namelin{} & 1.0 & \textbf{0.7} & \underline{6.2} & 112.3 & 0 \\
\bottomrule
\end{tabular*}
% \par\vspace{2pt}\begin{minipage}{\linewidth}\scriptsize Lower costs are better. \textbf{Bold}: best; \underline{underlined}: second distinct displayed value; ties share marks. A100 and CPU with twelve threads; batch one, $512\times384$ inputs; IEM uses $256\times256$. Peak GPU memory includes the model and inference temporaries. Our encoder costs exclude the pre-filter and output cosine. GFLOPs count visible tensor operations; human labels count similarity judgements.\end{minipage}
\end{table}
% ---- v23.7 wraptable version ----
% \begin{wraptable}[24]{r}{0.55\linewidth}
% \vspace{-12pt}
% \centering\scriptsize
% \captionsetup{font=footnotesize,skip=2pt}
% \caption{Cost per image pair. Violet: ours; grey: trained on human judgements.}
% \label{tab:app_cost}
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.03}
% % \caption{Cost per image pair. Violet: ours; grey: fitted on human judgements; white: other baselines.}  (moved beside the table)
% % \label{tab:app_cost}  (moved beside the table)
% \colorlet{humanJudgements}{gray!7}
% \definecolor{ourMetrics}{HTML}{F3EFF8}
% \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrr@{}}
% \toprule
% Metric & GFLOPs & GPU ms & CPU ms & \shortstack{Peak GPU\\MB} & Labels \\
% \midrule
% % Cell gflops_per_pair=10.7; exact=10.720791552; source: results/cost.csv:2, metric=jld, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=2.5; exact=2.525739546399564; source: results/cost.csv:2, metric=jld, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=29.8; exact=29.782272991724312; source: results/cost.csv:2, metric=jld, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=114.0; exact=113.99755859375; source: results/cost.csv:2, metric=jld, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:2, metric=jld, column=human_labels_used.
% \rowcolor{ourMetrics}\namefast{} & 10.7 & 2.5 & 29.8 & 114.0 & 0 \\
% % Cell gflops_per_pair=118.5; exact=118.467293184; source: results/cost.csv:3, metric=jld_full12, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=12.2; exact=12.249739957042038; source: results/cost.csv:3, metric=jld_full12, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=253.7; exact=253.668243996799; source: results/cost.csv:3, metric=jld_full12, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=115.4; exact=115.43505859375; source: results/cost.csv:3, metric=jld_full12, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:3, metric=jld_full12, column=human_labels_used.
% \rowcolor{ourMetrics}\name{} & 118.5 & 12.2 & 253.7 & 115.4 & 0 \\
% % Cell gflops_per_pair=$<$0.1; exact=0.0; source: results/cost.csv:4, metric=psnr, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=1.4; exact=1.4140065177343786; source: results/cost.csv:4, metric=psnr, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=1.1; exact=1.112711033783853; source: results/cost.csv:4, metric=psnr, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=9.0; exact=9.0; source: results/cost.csv:4, metric=psnr, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:4, metric=psnr, column=human_labels_used.
% PSNR & \textbf{$<$0.1} & \underline{1.4} & \textbf{1.1} & \textbf{9.0} & 0 \\
% % Cell gflops_per_pair=0.2; exact=0.234252968; source: results/cost.csv:5, metric=ssim, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=2.7; exact=2.678551943972707; source: results/cost.csv:5, metric=ssim, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=92.6; exact=92.56007801741362; source: results/cost.csv:5, metric=ssim, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=34.5; exact=34.529296875; source: results/cost.csv:5, metric=ssim, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:5, metric=ssim, column=human_labels_used.
% SSIM & \underline{0.2} & 2.7 & 92.6 & 34.5 & 0 \\
% % Cell gflops_per_pair=0.3; exact=0.303561768; source: results/cost.csv:6, metric=ms_ssim, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=5.1; exact=5.118806497193873; source: results/cost.csv:6, metric=ms_ssim, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=119.1; exact=119.14976697880776; source: results/cost.csv:6, metric=ms_ssim, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=34.5; exact=34.52978515625; source: results/cost.csv:6, metric=ms_ssim, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:6, metric=ms_ssim, column=human_labels_used.
% MS-SSIM & 0.3 & 5.1 & 119.1 & 34.5 & 0 \\
% % Cell gflops_per_pair=$<$0.1; exact=0.005308416; source: results/cost.csv:7, metric=fsim, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=22.8; exact=22.846897481940687; source: results/cost.csv:7, metric=fsim, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=60.6; exact=60.573618044145405; source: results/cost.csv:7, metric=fsim, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=46.2; exact=46.18798828125; source: results/cost.csv:7, metric=fsim, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:7, metric=fsim, column=human_labels_used.
% FSIM & \textbf{$<$0.1} & 22.8 & 60.6 & 46.2 & 0 \\
% % Cell gflops_per_pair=$<$0.1; exact=0.015335424; source: results/cost.csv:8, metric=vsi, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=9.9; exact=9.872902475763112; source: results/cost.csv:8, metric=vsi, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=39.8; exact=39.776562014594674; source: results/cost.csv:8, metric=vsi, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=48.7; exact=48.650390625; source: results/cost.csv:8, metric=vsi, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:8, metric=vsi, column=human_labels_used.
% VSI & \textbf{$<$0.1} & 9.9 & 39.8 & 48.7 & 0 \\
% % Cell gflops_per_pair=$<$0.1; exact=0.011403264; source: results/cost.csv:9, metric=gmsd, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=2.6; exact=2.5983754894696176; source: results/cost.csv:9, metric=gmsd, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=7.3; exact=7.331099011935294; source: results/cost.csv:9, metric=gmsd, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=18.6; exact=18.625; source: results/cost.csv:9, metric=gmsd, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:9, metric=gmsd, column=human_labels_used.
% GMSD & \textbf{$<$0.1} & 2.6 & 7.3 & \underline{18.6} & 0 \\
% % Cell gflops_per_pair=$<$0.1; exact=0.017856; source: results/cost.csv:10, metric=mad, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=247.9; exact=247.87814100272956; source: results/cost.csv:10, metric=mad, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=1,721.3; exact=1721.3351769605651; source: results/cost.csv:10, metric=mad, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=649.2; exact=649.15478515625; source: results/cost.csv:10, metric=mad, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:10, metric=mad, column=human_labels_used.
% MAD & \textbf{$<$0.1} & 247.9 & 1,721.3 & 649.2 & 0 \\
% % Cell gflops_per_pair=$<$0.1; exact=0.049952464; source: results/cost.csv:11, metric=nlpd, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=15.6; exact=15.560497005935758; source: results/cost.csv:11, metric=nlpd, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=27.1; exact=27.145628002472222; source: results/cost.csv:11, metric=nlpd, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=21.6; exact=21.60009765625; source: results/cost.csv:11, metric=nlpd, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:11, metric=nlpd, column=human_labels_used.
% NLPD & \textbf{$<$0.1} & 15.6 & 27.1 & 21.6 & 0 \\
% % Cell gflops_per_pair=1.7; exact=1.729021872; source: results/cost.csv:12, metric=vif, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=54.0; exact=53.98199800401926; source: results/cost.csv:12, metric=vif, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=126.6; exact=126.61413103342056; source: results/cost.csv:12, metric=vif, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=54.8; exact=54.83642578125; source: results/cost.csv:12, metric=vif, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:12, metric=vif, column=human_labels_used.
% VIF & 1.7 & 54.0 & 126.6 & 54.8 & 0 \\
% % Cell gflops_per_pair=240.6; exact=240.582918144; source: results/cost.csv:13, metric=lpips_vgg, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=10.9; exact=10.914095502812415; source: results/cost.csv:13, metric=lpips_vgg, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=418.5; exact=418.4992600930855; source: results/cost.csv:13, metric=lpips_vgg, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=532.3; exact=532.2646484375; source: results/cost.csv:13, metric=lpips_vgg, column=peak_gpu_MB.
% % Cell human_labels_used=484,000; exact=484000; source: results/cost.csv:13, metric=lpips_vgg, column=human_labels_used.
% \rowcolor{humanJudgements}LPIPS-VGG & 240.6 & 10.9 & 418.5 & 532.3 & 484,000 \\
% % Cell gflops_per_pair=10.9; exact=10.861507584; source: results/cost.csv:14, metric=lpips_alex, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=3.7; exact=3.676026011817157; source: results/cost.csv:14, metric=lpips_alex, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=34.1; exact=34.0727650327608; source: results/cost.csv:14, metric=lpips_alex, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=63.0; exact=63.02294921875; source: results/cost.csv:14, metric=lpips_alex, column=peak_gpu_MB.
% % Cell human_labels_used=484,000; exact=484000; source: results/cost.csv:14, metric=lpips_alex, column=human_labels_used.
% \rowcolor{humanJudgements}LPIPS-Alex & 10.9 & 3.7 & 34.1 & 63.0 & 484,000 \\
% % Cell gflops_per_pair=240.7; exact=240.747282432; source: results/cost.csv:15, metric=dists, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=9.9; exact=9.936597023624929; source: results/cost.csv:15, metric=dists, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=415.0; exact=415.02451710402966; source: results/cost.csv:15, metric=dists, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=340.7; exact=340.6953125; source: results/cost.csv:15, metric=dists, column=peak_gpu_MB.
% % Cell human_labels_used=484,000; exact=484000; source: results/cost.csv:15, metric=dists, column=human_labels_used.
% \rowcolor{humanJudgements}DISTS & 240.7 & 9.9 & 415.0 & 340.7 & 484,000 \\
% % Cell gflops_per_pair=385.7; exact=385.679253504; source: results/cost.csv:16, metric=pieapp, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=16.5; exact=16.537297051399946; source: results/cost.csv:16, metric=pieapp, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=797.0; exact=797.0107579603791; source: results/cost.csv:16, metric=pieapp, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=1,005.5; exact=1005.51123046875; source: results/cost.csv:16, metric=pieapp, column=peak_gpu_MB.
% % Cell human_labels_used=2,300,000; exact=2300000; source: results/cost.csv:16, metric=pieapp, column=human_labels_used.
% \rowcolor{humanJudgements}PieAPP & 385.7 & 16.5 & 797.0 & 1,005.5 & 2,300,000 \\
% % Cell gflops_per_pair=326.4; exact=326.356697088; source: results/cost.csv:17, metric=deepdc, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=16.1; exact=16.072013997472823; source: results/cost.csv:17, metric=deepdc, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=509.6; exact=509.5683719264344; source: results/cost.csv:17, metric=deepdc, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=325.2; exact=325.15478515625; source: results/cost.csv:17, metric=deepdc, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:17, metric=deepdc, column=human_labels_used.
% DeepDC & 326.4 & 16.1 & 509.6 & 325.2 & 0 \\
% % Cell gflops_per_pair=212.2; exact=212.154212352; source: results/cost.csv:18, metric=dreamsim, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=51.3; exact=51.26894399290904; source: results/cost.csv:18, metric=dreamsim, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=549.6; exact=549.6234609745443; source: results/cost.csv:18, metric=dreamsim, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=1,041.9; exact=1041.8583984375; source: results/cost.csv:18, metric=dreamsim, column=peak_gpu_MB.
% % Cell human_labels_used=20,000; exact=20000; source: results/cost.csv:18, metric=dreamsim, column=human_labels_used.
% \rowcolor{humanJudgements}DreamSim & 212.2 & 51.3 & 549.6 & 1,041.9 & 20,000 \\
% % Cell gflops_per_pair=60.2; exact=60.189179904; source: results/cost.csv:19, metric=deepwsd, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=13.5; exact=13.5155440075323; source: results/cost.csv:19, metric=deepwsd, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=442.6; exact=442.63165502343327; source: results/cost.csv:19, metric=deepwsd, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=709.3; exact=709.29443359375; source: results/cost.csv:19, metric=deepwsd, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:19, metric=deepwsd, column=human_labels_used.
% DeepWSD & 60.2 & 13.5 & 442.6 & 709.3 & 0 \\
% % Cell gflops_per_pair=0.3; exact=0.339738624; source: results/cost.csv:20, metric=lasi, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=377.6; exact=377.6092884945683; source: results/cost.csv:20, metric=lasi, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=13,554.5; exact=13554.450307041408; source: results/cost.csv:20, metric=lasi, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=2,683.7; exact=2683.68896484375; source: results/cost.csv:20, metric=lasi, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:20, metric=lasi, column=human_labels_used.
% LASI & 0.3 & 377.6 & 13,554.5 & 2,683.7 & 0 \\
% % Cell gflops_per_pair=4,999.1; exact=4999.11643136; source: results/cost.csv:21, metric=iem, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=725.7; exact=725.7345230318606; source: results/cost.csv:21, metric=iem, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=22,766.5; exact=22766.52321300935; source: results/cost.csv:21, metric=iem, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=5,434.2; exact=5434.16259765625; source: results/cost.csv:21, metric=iem, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost.csv:21, metric=iem, column=human_labels_used.
% IEM & 4,999.1 & 725.7 & 22,766.5 & 5,434.2 & 0 \\
% % Cell gflops_per_pair=1.0; exact=0.973430784; source: results/cost_tiers.csv:2, metric=jld_lin, column=gflops_per_pair.
% % Cell gpu_ms_per_pair=0.7; exact=0.6615369929932058; source: results/cost_tiers.csv:2, metric=jld_lin, column=gpu_ms_per_pair.
% % Cell cpu_ms_per_pair=6.2; exact=6.238780915737152; source: results/cost_tiers.csv:2, metric=jld_lin, column=cpu_ms_per_pair.
% % Cell peak_gpu_MB=112.3; exact=112.30224609375; source: results/cost_tiers.csv:2, metric=jld_lin, column=peak_gpu_MB.
% % Cell human_labels_used=0; exact=0; source: results/cost_tiers.csv:2, metric=jld_lin, column=human_labels_used.
% \rowcolor{ourMetrics}\namelin{} & 1.0 & \textbf{0.7} & \underline{6.2} & 112.3 & 0 \\
% \bottomrule
% \end{tabular*}
% % \par\vspace{2pt}\begin{minipage}{\linewidth}\scriptsize Lower costs are better. \textbf{Bold}: best; \underline{underlined}: second distinct displayed value; ties share marks. A100 and CPU with twelve threads; batch one, $512\times384$ inputs; IEM uses $256\times256$. Peak GPU memory includes the model and inference temporaries. Our encoder costs exclude the pre-filter and output cosine. GFLOPs count visible tensor operations; human labels count similarity judgements.\end{minipage}
% {\scriptsize\par\vspace{2pt} A100 and twelve CPU threads, batch one, $512\times384$ inputs (IEM $256\times256$). \name{} timings exclude the pre-filter and output cosine.\par}
% \vspace{-10pt}
% \end{wraptable}
% v23.5 side-caption block, replaced in v23.6:
% \end{minipage}\hfill
% \begin{minipage}[c]{0.35\linewidth}
% \caption{Cost per image pair. Violet: ours; grey: fitted on human judgements; white: other baselines.}
% \label{tab:app_cost}
% {\scriptsize Lower costs are better. \textbf{Bold}: best; \underline{underlined}: second distinct displayed value; ties share marks. A100 and CPU with twelve threads; batch one, $512\times384$ inputs; IEM uses $256\times256$. Peak GPU memory includes the model and inference temporaries. Our encoder costs exclude the pre-filter and output cosine. GFLOPs count visible tensor operations; human labels count similarity judgements.}
% \end{minipage}
% \end{table}


==> tables/app_mechanism.tex <==
% Generated by scripts/v18/tables.py; numeric receipts in docs/presentation-v18/new-tables.json.
\begin{table}[!ht]% v23.6 P6: was [tbp]
\centering\footnotesize% v23.5 P2: was \small
\setlength{\tabcolsep}{3pt}
% \caption{Type-level Spearman correlation between blindness and human tolerance after controlling raw feature distance (left), and the predefined lens sensitivity checks (right). Random averages five fixed seeds; P2 correlates reference-demeaned blindness with rank-error gain.}
\caption{Type-level Spearman correlation between blindness and human tolerance after controlling raw feature distance (left), and the predefined sensitivity checks (right). P2: reference-demeaned blindness against rank-error gain.}
\label{tab:mechanism}\label{tab:mechanism-sensitivity}
% Point estimates from the v18 tables mechanism and mechanism_sensitivity (values unchanged; intervals omitted).
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrrrr@{}}
\toprule
 & \multicolumn{4}{c}{Raw-distance control} & \multicolumn{4}{c}{Lens sensitivity checks} \\
\cmidrule(lr){2-5}\cmidrule(l){6-9}
Dataset & Lens & PCA & Random & Lens$-$PCA & PSNR ctrl. & Energy & Nonchrom. & P2 gain \\
\midrule
KADID dev & $0.633$ & $0.325$ & $-0.073$ & $0.308$ & $-0.253$ & $0.726$ & $0.387$ & $0.124$ \\
KADID test & $0.655$ & $0.363$ & $0.028$ & $0.292$ & $-0.302$ & $0.679$ & $0.412$ & $0.112$ \\
LIVE & $0.500$ & $0.600$ & $0.300$ & $-0.100$ & $0.100$ & $0.500$ & $0.500$ & $0.035$ \\
TID2013 diag. & $0.725$ & $0.613$ & $0.046$ & $0.112$ & $0.325$ & $0.731$ & $0.741$ & $-0.073$ \\
\bottomrule
\end{tabular*}
\end{table}


==> tables/app_quality_transfer.tex <==
% Generated by scripts/v15/results.py from audited CSVs; do not edit by hand.
\begin{table}[!htbp]
\centering\footnotesize% v23.5 P2: was \small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.0}% v23.5 P2: was 1.12
\definecolor{qualityLens}{HTML}{F3EFF8}
% \caption{Signed SRCC of TOPIQ-NR outputs, feature controls and Quality JLD on all 4,645 image pairs (779 LIVE, 866 CSIQ and 3,000 TID2013, grouped by 29, 30 and 25 references). Quality JLD gives mixed gains over the matched controls.}
\caption{Signed \srcc{} of TOPIQ-NR outputs, feature controls and Quality \name{} on 4{,}645 image pairs of LIVE, CSIQ and TID2013. ``Within'' averages per-reference correlations; ``Random'' averages five projections.}
\label{tab:quality-transfer}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrr@{}}
\toprule
 & \multicolumn{2}{c}{LIVE} & \multicolumn{2}{c}{CSIQ} & \multicolumn{2}{c}{TID2013} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Method & Pooled & Within & Pooled & Within & Pooled & Within \\
\midrule
% Cell 0.835; exact=0.8346015205452768; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:2, column=pooled_srcc.
% Cell 0.840; exact=0.8403513175513614; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:2, column=mean_within_source_srcc.
% Cell 0.748; exact=0.7478029732084843; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:22, column=pooled_srcc.
% Cell 0.820; exact=0.819745432262929; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:22, column=mean_within_source_srcc.
% Cell 0.445; exact=0.4452100846302179; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:42, column=pooled_srcc.
% Cell 0.485; exact=0.4846442520861114; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:42, column=mean_within_source_srcc.
Original NR head & 0.835 & 0.840 & 0.748 & 0.820 & 0.445 & 0.485 \\
% Cell 0.833; exact=0.8331490414308039; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:3, column=pooled_srcc.
% Cell 0.840; exact=0.8403513175513614; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:3, column=mean_within_source_srcc.
% Cell 0.801; exact=0.8006413650526443; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:23, column=pooled_srcc.
% Cell 0.820; exact=0.819745432262929; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:23, column=mean_within_source_srcc.
% Cell 0.454; exact=0.45373019126451064; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:43, column=pooled_srcc.
% Cell 0.485; exact=0.4846442520861114; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:43, column=mean_within_source_srcc.
Signed score drop & 0.833 & 0.840 & 0.801 & 0.820 & 0.454 & 0.485 \\
% Cell 0.833; exact=0.8328714105027033; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:4, column=pooled_srcc.
% Cell 0.839; exact=0.8393853895655424; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:4, column=mean_within_source_srcc.
% Cell 0.793; exact=0.7934435473693049; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:24, column=pooled_srcc.
% Cell 0.809; exact=0.8090055258949337; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:24, column=mean_within_source_srcc.
% Cell 0.445; exact=0.4445969187377968; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:44, column=pooled_srcc.
% Cell 0.474; exact=0.4735427351974302; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:44, column=mean_within_source_srcc.
Absolute score gap & 0.833 & 0.839 & 0.793 & 0.809 & 0.445 & 0.474 \\
\addlinespace[3pt]
% Cell 0.873; exact=0.8729706615029791; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:20, column=pooled_srcc.
% Cell 0.927; exact=0.9272883667717535; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:20, column=mean_within_source_srcc.
% Cell 0.809; exact=0.8086909105297525; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:40, column=pooled_srcc.
% Cell 0.832; exact=0.8317385461005559; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:40, column=mean_within_source_srcc.
% Cell 0.687; exact=0.6869112699099483; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:60, column=pooled_srcc.
% Cell 0.692; exact=0.6915373546469613; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:60, column=mean_within_source_srcc.
Pixel RMSE & 0.873 & 0.927 & 0.809 & 0.832 & 0.687 & 0.692 \\
\addlinespace[3pt]
% Cell 0.924; exact=0.9239003386439967; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:5, column=pooled_srcc.
% Cell 0.939; exact=0.9394688363576236; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:5, column=mean_within_source_srcc.
% Cell 0.858; exact=0.8583627324034404; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:25, column=pooled_srcc.
% Cell 0.868; exact=0.8679292710690624; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:25, column=mean_within_source_srcc.
% Cell 0.673; exact=0.6725610705482724; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:45, column=pooled_srcc.
% Cell 0.675; exact=0.6745727226180471; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:45, column=mean_within_source_srcc.
Raw features (256) & 0.924 & 0.939 & 0.858 & 0.868 & 0.673 & 0.675 \\
% Cell 0.934; exact=0.9337131464262327; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:8, column=pooled_srcc.
% Cell 0.943; exact=0.9433711088558541; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:8, column=mean_within_source_srcc.
% Cell 0.861; exact=0.8609901695439403; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:28, column=pooled_srcc.
% Cell 0.869; exact=0.8685659939401246; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:28, column=mean_within_source_srcc.
% Cell 0.685; exact=0.685247122490908; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:48, column=pooled_srcc.
% Cell 0.689; exact=0.6887829500070076; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:48, column=mean_within_source_srcc.
PCA (64) & 0.934 & 0.943 & 0.861 & 0.869 & 0.685 & 0.689 \\
% Cell 0.925; exact=0.9246485333163081; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:21, column=pooled_srcc.
% Cell 0.941; exact=0.9405475173201345; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:21, column=mean_within_source_srcc.
% Cell 0.859; exact=0.8590150505384144; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:41, column=pooled_srcc.
% Cell 0.868; exact=0.8680772066322265; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:41, column=mean_within_source_srcc.
% Cell 0.671; exact=0.6708114669708314; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:61, column=pooled_srcc.
% Cell 0.674; exact=0.6735852413869562; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:61, column=mean_within_source_srcc.
Random (64; 5 seeds) & 0.925 & 0.941 & 0.859 & 0.868 & 0.671 & 0.674 \\
% Cell 0.927; exact=0.9269989811018486; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:12, column=pooled_srcc.
% Cell 0.940; exact=0.9398938433112245; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:12, column=mean_within_source_srcc.
% Cell 0.865; exact=0.8654628998841621; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:32, column=pooled_srcc.
% Cell 0.870; exact=0.8695977349154067; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:32, column=mean_within_source_srcc.
% Cell 0.680; exact=0.6797477783724067; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:52, column=pooled_srcc.
% Cell 0.682; exact=0.6815956875773699; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:52, column=mean_within_source_srcc.
\rowcolor{qualityLens}Quality JLD (64) & 0.927 & 0.940 & 0.865 & 0.870 & 0.680 & 0.682 \\
\addlinespace[3pt]
% Cell 0.976; exact=0.9758960976462332; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:19, column=pooled_srcc.
% Cell 0.977; exact=0.9768874743829203; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:19, column=mean_within_source_srcc.
% Cell 0.967; exact=0.9674094342641516; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:39, column=pooled_srcc.
% Cell 0.971; exact=0.9714687670027568; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:39, column=mean_within_source_srcc.
% Cell 0.917; exact=0.9165426346388442; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:59, column=pooled_srcc.
% Cell 0.934; exact=0.9342450530271234; scale=1; source: docs/quality-encoder-pilot/signed-correlations.csv:59, column=mean_within_source_srcc.
Published TOPIQ-FR & 0.976 & 0.977 & 0.967 & 0.971 & 0.917 & 0.934 \\
\bottomrule
\end{tabular*}
% \par\vspace{3pt}\begin{minipage}{\linewidth}\footnotesize Higher is better. Within: equal-weight mean of per-reference SRCCs. Random: mean of five separately computed correlations. All feature controls use the same frozen KonIQ-trained TOPIQ-NR checkpoint and native RGB pairs. The last row is a separate KADID-trained reference-based checkpoint (TOPIQ-FR). These are previously used project benchmarks, not untouched project-wide holdouts.\end{minipage}
% v23.6 P6: shorter note.
\end{table}


==> tables/app_quality_transfer_uncertainty.tex <==
% Generated by scripts/v15/results.py from audited CSVs (docs/quality-encoder-pilot/paired-source-bootstrap.csv, v16 table);
% v23.3 (D2): transposed into a narrow wraptable, values rounded to three decimals from the CSV; intervals omitted.
\begin{wraptable}{r}{0.42\linewidth}
\vspace{-12pt}
\centering\small
\setlength{\tabcolsep}{3pt}
\caption{Quality JLD minus each same-checkpoint TOPIQ control (SRCC). Every gap is below 0.01.}
\label{tab:quality-transfer-uncertainty}
\begin{tabular}{@{}llrrr@{}}
\toprule
 & & Raw & PCA & Random \\
\midrule
LIVE & pooled & $+0.003$ & $-0.007$ & $+0.002$ \\
 & within & $+0.000$ & $-0.003$ & $-0.001$ \\
CSIQ & pooled & $+0.007$ & $+0.004$ & $+0.006$ \\
 & within & $+0.002$ & $+0.001$ & $+0.002$ \\
TID & pooled & $+0.007$ & $-0.005$ & $+0.009$ \\
 & within & $+0.007$ & $-0.007$ & $+0.008$ \\
\bottomrule
\end{tabular}
\vspace{-8pt}
\end{wraptable}


==> tables/app_quality_video_transfer.tex <==
% Generated by scripts/v15/results.py from audited CSVs; do not edit by hand.
\begin{table}[!htbp]
\centering\footnotesize% v23.5 P2: was \small
\setlength{\tabcolsep}{3pt}
\definecolor{qualityLens}{HTML}{F3EFF8}
% \caption{DOVER technical-branch transfer on all 120 AVT test-1 clips, with a fixed 32-frame sample per source. Pooled SRCC, source-mean SRCC and pair agreement rank the methods differently; the last four columns give signed SRCC over the 30 clips of each source.}
\caption{DOVER technical-branch transfer on the 120 AVT test-1 clips. The last four columns give signed \srcc{} over the 30 clips of each source. Pair agreement uses within-source pairs with nonoverlapping MOS intervals.}
\label{tab:quality-video-transfer}\label{tab:quality-video-sources}
% Merged from the v16 tables quality_video_transfer and quality_video_sources (values unchanged).
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrrr@{}}
\toprule
 & \multicolumn{3}{c}{All clips} & \multicolumn{4}{c}{Per source} \\
\cmidrule(lr){2-4}\cmidrule(l){5-8}
Method & Pooled & Src.\ mean & Pairs (\%) & Anim. & Orange & Veg. & Water \\
\midrule
NR head: native input & 0.6977 & 0.6999 & 89.40 & 0.9753 & 0.2199 & 0.7679 & 0.8365 \\
\addlinespace[3pt]
NR head: matched input & 0.8706 & 0.9167 & 96.81 & 0.9757 & 0.9121 & 0.9410 & 0.8379 \\
Signed score drop & 0.8784 & 0.9167 & 96.81 & 0.9757 & 0.9121 & 0.9410 & 0.8379 \\
Absolute score gap & 0.8598 & 0.8530 & 95.78 & 0.9757 & 0.7521 & 0.8464 & 0.8379 \\
\addlinespace[3pt]
Raw features (96) & 0.6830 & 0.8516 & 97.16 & 0.9791 & 0.8769 & 0.5900 & 0.9605 \\
PCA (32) & 0.6921 & 0.8575 & 97.24 & 0.9791 & 0.8916 & 0.5923 & 0.9670 \\
Random (32; 5 seeds) & 0.6831 & 0.8556 & 97.22 & 0.9784 & 0.8817 & 0.5986 & 0.9638 \\
\rowcolor{qualityLens}Quality JLD (32) & 0.7062 & 0.8968 & 98.53 & 0.9795 & 0.9197 & 0.7138 & 0.9743 \\
\bottomrule
\end{tabular*}
% \par\vspace{3pt}\begin{minipage}{\linewidth}\footnotesize Matched input scores the same distorted fragments from a common UHD canvas as the reference-based methods; native input keeps stored resolution. Pair agreement uses the 1,160 within-source pairs with nonoverlapping MOS intervals. Random averages five separate statistics. This is not the official fused, three-clip DOVER protocol.\end{minipage}
% v23.6 P6: shorter note.
\end{table}


==> tables/app_types_merged.tex <==
% v23.5 P2: merged from tables/app_types_tid2013.tex and tables/app_types_kadid10k_test.tex (final-comparison
% columns copied cell for cell by a script, marks included; the "Original" Ref./CLS columns are dropped here and remain in
% the two source tables, which are no longer input).
\begin{table}[!tb]
\centering\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.0}
\caption{\srcc{} by distortion type on TID2013 (diagnostic) and KADID-10k test. Violet: ours; grey: fitted on human judgements; white: other baselines. Higher is better; \textbf{bold} and \underline{underlining} mark the best and second distinct displayed values within each type, with ties sharing marks.}
\label{tab:app_types_tid2013}\label{tab:app_types_kadid10k_test}\label{tab:app_types_merged}
\colorlet{humanJudgements}{gray!7}
\definecolor{ourMetrics}{HTML}{F3EFF8}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}rl>{\columncolor{ourMetrics}}r>{\columncolor{humanJudgements}}rrrl>{\columncolor{ourMetrics}}r>{\columncolor{humanJudgements}}rrr@{}}
\toprule
& \multicolumn{5}{c}{TID2013} & \multicolumn{5}{c}{KADID-10k test} \\
\cmidrule(lr){2-6}\cmidrule(l){7-11}
ID & Distortion & \name{} & DISTS & VSI & DeepWSD & Distortion & \name{} & DISTS & VSI & DeepWSD \\
\midrule
1 & additive Gaussian noise & 0.916 & 0.855 & \textbf{0.945} & \underline{0.938} & Gaussian blur & 0.947 & \textbf{0.963} & \underline{0.956} & 0.939 \\
2 & noise in colour components & 0.843 & 0.805 & \textbf{0.866} & \underline{0.851} & lens blur & \underline{0.912} & \textbf{0.938} & 0.907 & 0.848 \\
3 & spatially correlated noise & 0.926 & 0.863 & \underline{0.934} & \textbf{0.936} & motion blur & 0.938 & \textbf{0.962} & \underline{0.953} & 0.931 \\
4 & masked noise & \underline{0.823} & 0.813 & 0.769 & \textbf{0.837} & colour diffusion & \textbf{0.925} & 0.887 & \underline{0.916} & 0.883 \\
5 & high-frequency noise & 0.892 & 0.866 & \textbf{0.920} & \underline{0.909} & colour shift & \underline{0.802} & \textbf{0.882} & 0.790 & 0.720 \\
6 & impulse noise & 0.792 & 0.707 & \textbf{0.875} & \underline{0.829} & colour quantisation & \textbf{0.888} & 0.844 & \underline{0.857} & 0.848 \\
7 & quantisation noise & \underline{0.883} & 0.819 & 0.868 & \textbf{0.900} & colour saturation 1 & \textbf{0.682} & \underline{0.668} & 0.627 & 0.614 \\
8 & Gaussian blur & 0.928 & 0.936 & \textbf{0.966} & \underline{0.965} & colour saturation 2 & \underline{0.932} & 0.926 & \textbf{0.939} & 0.914 \\
9 & image denoising & 0.935 & 0.899 & \textbf{0.945} & \underline{0.939} & JPEG2000 & \underline{0.945} & \textbf{0.946} & 0.939 & 0.929 \\
10 & JPEG & 0.932 & 0.898 & \textbf{0.957} & \underline{0.954} & JPEG & \underline{0.869} & \textbf{0.884} & 0.864 & 0.811 \\
11 & JPEG2000 & 0.960 & 0.941 & \textbf{0.971} & \underline{0.963} & white noise & 0.903 & 0.859 & \underline{0.920} & \textbf{0.922} \\
12 & JPEG transmission errors & \underline{0.921} & \textbf{0.924} & 0.920 & \textbf{0.924} & white noise in colour & 0.941 & 0.907 & \textbf{0.951} & \underline{0.942} \\
13 & JPEG2000 transmission errors & 0.921 & 0.866 & \underline{0.923} & \textbf{0.943} & impulse noise & 0.897 & 0.823 & \textbf{0.913} & \underline{0.899} \\
14 & non-eccentricity pattern noise & \underline{0.825} & \textbf{0.841} & 0.802 & 0.824 & multiplicative noise & \underline{0.956} & 0.908 & 0.953 & \textbf{0.958} \\
15 & local block-wise distortions & \underline{0.515} & 0.350 & 0.160 & \textbf{0.573} & denoising & \underline{0.906} & \textbf{0.926} & 0.867 & 0.841 \\
16 & mean shift & \textbf{0.810} & \underline{0.809} & 0.774 & 0.740 & brighten & \underline{0.935} & \textbf{0.946} & 0.912 & 0.911 \\
17 & contrast change & 0.378 & \textbf{0.483} & \underline{0.476} & 0.459 & darken & \underline{0.907} & \textbf{0.917} & 0.905 & 0.888 \\
18 & colour saturation change & \textbf{0.858} & 0.810 & 0.811 & \underline{0.832} & mean shift & \underline{0.735} & \textbf{0.780} & 0.701 & 0.676 \\
19 & multiplicative Gaussian noise & 0.875 & 0.810 & \textbf{0.908} & \underline{0.897} & jitter & \underline{0.952} & \textbf{0.963} & 0.949 & 0.944 \\
20 & comfort noise & 0.921 & 0.892 & \underline{0.925} & \textbf{0.933} & non-eccentricity patch & 0.471 & \textbf{0.644} & \underline{0.494} & 0.444 \\
21 & lossy compression of noisy images & \textbf{0.963} & 0.934 & 0.955 & \underline{0.956} & pixelate & \underline{0.612} & \textbf{0.813} & 0.546 & 0.583 \\
22 & colour quantisation with dither & \underline{0.902} & 0.868 & 0.881 & \textbf{0.909} & quantisation & \underline{0.810} & \textbf{0.872} & 0.673 & 0.751 \\
23 & chromatic aberrations & 0.885 & \textbf{0.895} & \underline{0.890} & \textbf{0.895} & colour block & \underline{0.594} & \textbf{0.601} & 0.472 & 0.585 \\
24 & sparse sampling and reconstruction & \underline{0.960} & 0.951 & \textbf{0.963} & 0.949 & high sharpen & \underline{0.895} & 0.891 & \textbf{0.919} & 0.882 \\
25 & & & & & & contrast change & 0.687 & \textbf{0.773} & \underline{0.750} & 0.672 \\
\bottomrule
\end{tabular*}
\end{table}

